Your Eyes Say You're Lying: An Eye Movement Pattern Analysis for Face Familiarity and Deceptive Cognition

Eye movement patterns reflect human latent internal cognitive activities. We aim to discover eye movement patterns during face recognition under different cognitions of information concealing. These cognitions include the degrees of face familiarity and deception or not, namely telling the truth when observing familiar and unfamiliar faces, and deceiving in front of familiar faces. We apply Hidden Markov models with Gaussian emission to generalize regions and trajectories of eye fixation points under the above three conditions. Our results show that both eye movement patterns and eye gaze regions become significantly different during deception compared with truth-telling. We show the feasibility of detecting deception and further cognitive activity classification using eye movement patterns.

==> secs/discussion.tex <==
\section{Discussion}

\subsection{Estimating Our Proposed Model}

Given the transition and the emission matrices we generated for each representative model,
we can calculate the Viterbi path of the states the model would most likely go through. In this section, we will randomly pick some real eye movement sequence from our participants, and fit them into the obtained representative models and compute the percentage of the actual eye movement sequence that agrees with the likely states sequence. And we consider the model with the highest probability to be the cluster the eye movement sequence belongs to. To test the accuracy of the model classification, for each participant, we consider three typical eye
movement data that generate from conditions of telling-truth-on-familiar- faces, telling-truth- on-unfamiliar-faces, and lying-on-familiar-faces separately to be the testing set. The total number of the testing eye movement sequence is sixty-three.
17 out of 21 participants (i.e. 80.95\%) of telling-truth-on-familiar-face patterns are classified to correct cluster, 4 of the incorrect ones are classified to the telling-truth-on-unfamiliar faces.
13 out of 21 participants (i.e. 61.90\%) of telling-truth-on-unfamiliar-face patterns are
classified to correct cluster, 4 of the incorrect ones are classified to the lying-on-familiar-faces, 3 of the incorrect ones are classified to the telling-truth--on-familiar-faces.
17 out of 21 participants (i.e. 80.95\%) of lying-on-familiar-face patterns are classified to correct cluster, 2 of the incorrect ones are classified to the telling-truth-on-familiar-faces, 2 of the incorrect ones are classified to the telling-truth-on-unfamiliar-faces.
The accuracy of all the three circumstances are well above chance. The results show that the eye movement patterns when people are looking at familiar faces are consistent, as the accuracy of classification are both high in telling-truth-on-familiar-face and lying-on-familiar-face conditions. When people are looking at unfamiliar faces, the eye movement pattern is less consistent among different people but the accuracy is still close to double chance.

\subsection{Some Discussion}

We found that the general eye movement patterns in the condition of telling-truth-on-familiar- faces, telling-truth-on-unfamiliar-faces, and lying-on-familiar-faces has significant differences in not only the ROI location and area, but also the transition probabilities and time sequence of ROI.
When the participants are lying about their familiarity level of the viewed face, the ROIs tend to locate on the central axis of the face from top to bottom. When the participants are telling truth about the faces, the ROIs tend to locate at regions close to the two eyes and the region covers nose and mouth, which is an approximate triangle with its vertex composed by the three regions as described.
Differences between telling the truth about the familiarity level while viewing familiar and unfamiliar faces can be observed in the time order of the ROI sequence. Both of the eye movement patterns tend to start from the upper part of the face, while for the first situation, the scan path is most likely to start from the left eye from observer perspective, and for the second one, the initial fixation tend to locate at the right eye, again, from observer perspective. The most likely subsequent paths are also different, strategy for viewing familiar face is moving in between the two eye regions from observer perspective (remain or move back and forth); strategy for viewing unfamiliar face is moving in between the left eye region and the lower part of the face, still, from observer perspective (remain or move back and forth). Nevertheless, differences between the third case and the first two cases is quite obvious, however, it seems like that the general ROI of the first and second cases are similar (i.e. A general triangular path consisting of two eyes and the tip of the nose), and the range can not be a distinct characteristic to distinguish from each other.
In addition, during the real-world investigation, we can find the difference not only exists in time order of the states sequence from the transition probabilities, but also in the way fixations distribute. As can be seen from the Table 5.4 and 5.5, the representative ROI clustering centers of the first and second case are:
Case 1 (634.9725, 351.6586) (676.1114, 493.2836) (706.2081, 332.5524) Case 2 (672.2400, 430.2586) (616.2596, 321.0105) (688.8656, 337.2602) And the center of the face should be at (683, 384), by calculating the variance between the ROI clustering centers and the face center, the value of case 2 is significantly lower than the value of case 1, both on x and y dimension. Thus, we can infer that when people are viewing an unfamiliar face, the eye gaze can be more focused on the internal region of the face.

==> secs/related_work.tex <==
\section{Related Work}

In this section, we discuss some related previous important works in order to help readers understanding. 



Facial appearance is a highly sensitive area, which is essential for human identification and
communication. The ability of facial recognition is an essential human skill that can efficiently extract information such as gender, emotional situation, and familiarity. And the most important clue that can be obtained from face recognition is human identity. Previous studies show that recognition for familiar faces is more rapid and accurate compared with unfamiliar faces, allowing memories of a person to be accessed~\cite{stacey2005face}. Sometimes people are able to recognize the face they familiar with even in photos with very low quality, but are quite error prone when recognizing unfamiliar faces, which suggests differential treatment for familiar and unfamiliar faces. A simplified explanation is that familiar and unfamiliar face recognition is performed through independent, separate routes and distinct codes.

During the process of face recognition, in most cases, the first task people perform is to determine whether the face is familiar or unfamiliar. One interesting point to note is that people can almost instantly figure out if the face is familiar to them or not. The reason we make such quick decisions is because we divide the human face into internal and external region unconsciously, which helps us to automatically recognize a known face, or figure out an unfamiliar face. Internal features account for 31\% of the total face comprising the eyes, nose and mouth region, while the remaining parts of the face are classified as external features, that constitute about 69\% of the total area of the face. It has been reported that when the internal region of a familiar face is shown, observers’ response time were shorter than when the external region were shown~\cite{bruce1986understanding}.

Recent studies suggest that eye movement has functional roles and can reflect the underlying cognitive processes in face recognition. For example, it is shown that when observer were required to focus only at the center of a face images, their recognition ability can be significantly lower than when looking at face images freely~\cite{henderson2005eye}. Hsiao and Cottrell (2008) has found that two fixation points were sufficient for face recognition, and the points are located around the nose region, which suggests the preferred fixated location in face recognition. Fixated location has also been observed in the other cognitive processes in eye movement including driving, reading and video viewing. These finding show that a fixation in face recognition tasks play functional roles and are not randomly selected.
